KnowRL: Exploring Knowledgeable Reinforcement Learning for Factuality

Large Language Models (LLMs), particularly slow-thinking models, often exhibit severe hallucination, outputting incorrect content due to an inability to accurately recognize knowledge boundaries during reasoning. While Reinforcement Learning (RL) can enhance complex reasoning abilities, its outcome-oriented reward mechanism often lacks factual supervision over the thinking process, further exacerbating the hallucination problem. To address the high hallucination in slow-thinking models, we propose Knowledge-enhanced RL, KnowRL. KnowRL guides models to perform fact-based slow thinking by integrating a factuality reward, based on knowledge verification, into the RL training process, helping them recognize their knowledge boundaries. KnowRL guides models to perform fact-based slow thinking by integrating a factuality reward, based on knowledge verification, into the RL training process, helping them recognize their knowledge boundaries. This targeted factual input during RL training enables the model to learn and internalize fact-based reasoning strategies. By directly rewarding adherence to facts within the reasoning steps, KnowRL fosters a more reliable thinking process. Experimental results on three hallucination evaluation datasets and two reasoning evaluation datasets demonstrate that KnowRL effectively mitigates hallucinations in slow-thinking models while maintaining their original strong reasoning capabilities. Our code is available at https://github.com/zjunlp/KnowRL.

==> section_knowrl/Hallucination_in_st.tex <==




\section{Hallucination in Slow-thinking Models}

% \begin{tcolorbox}[colback=gray!5,colframe=gray!40!black,title=Definition]
% \textbf{Slow-thinking models} refer to language models that solve tasks via explicit multi-step reasoning. 
% This design enhances their ability to decompose complex problems but simultaneously increases exposure to factual errors, as inaccuracies may propagate across reasoning steps.
% \end{tcolorbox}


While slow-thinking models provide structured reasoning, they also amplify the risk of hallucinations. 
Figure~\ref{fig:scaling} illustrates this trade-off: larger DeepSeek-R1-Distill models achieve higher GPQA scores (reasoning ability) but fail to improve on SimpleQA (hallucination resistance), showing that scaling strengthens reasoning without resolving factual reliability issues.

\begin{definitionbox}
\textbf{The Hallucination Challenge in Slow-Thinking Models.} The multi-step reasoning of slow-thinking models creates a critical vulnerability to error propagation, where an initial factual inaccuracy cascades through the reasoning chain to yield a conclusion that is logically coherent but factually ungrounded.
\end{definitionbox}

The root cause lies in the factual supervision gap within current training paradigms. Existing approaches often emphasize reproducing reasoning patterns or final outcomes without verifying the factual accuracy of intermediate reasoning steps, leading models to generate coherent yet factually unsupported chains of thought.
Consequently, models may generate reasoning chains that sound coherent but are factually ungrounded, as evidenced by prior work \citep{heyman2025reasoning,patel2024multi,arcuschin2025chain}. 

This gap also explains why outcome-based RL is insufficient: rewarding only final correctness neglects factual consistency during reasoning. 
Worse, it may reinforce “lucky” but unreliable chains. 
Thus, mitigating hallucinations in slow-thinking models requires training strategies that directly enforce factual grounding—an objective we address with KnowRL.

% We use SimpleQA, TruthfulQA and ChineseSimpleQA datasets as the hallucination evaluation datasets, and GPQA dataset as the dataset for evaluating the model's reasoning ability. 



% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{images/slow-thinking.pdf}
%     % \vspace{-2ex}
%     \caption{Accuracy of the slow thinking model on the GPQA dataset.}
%     \vspace{-3ex}
%     \label{slow-thinking-gpqa}
% \end{figure}







==> section_knowrl/data.tex <==
\section{Data Construction} %%%%%%%%%%%%%%%%%%%%%

In large-scale training, redundant information increases storage and computation costs and affects the performance of RL training. 
To ensure the quality of the training data for RL, we screen high-quality Q\&A data from several open-source datasets for training and use DeepSeek-R1 to obtain long COT data for SFT. The following are data construction steps.

\subsection{RL Data Construction}
 We use part of the data extracted from NqOpen \cite{kwiatkowski2019natural,lee2019latent}, WebQuestions \citep{berant2013semantic}, and ComplexQuestions \citep{bao2016constraint} as factual question data sources.

\paragraph{Pre-processing and Simple Filtering.}
First of all, we filter out data that has multiple possible answers. 
This is because data with non-unique answers can easily lead to unstable training. 
At the same time, we filtered out the data with no obvious questioning tone in the questions, as such data can easily lead to the model not knowing the meaning of the question and thus blindly exploring it during the training process, thus affecting the training performance. 
We believe that there is no need for RL training for simple questions, so we use the Qwen2.5-7B-Instruct \citep{qwen2.5} to filter the simple data in the data source, and the filtering method is to filter out the questions that are answered correctly for the first time by the Qwen2.5-7B-Instruct.

\paragraph{Multiple De-duplication and Entropy Filtering.}
We decided to de-duplicate the data of NqOpen due to its large amount and not strictly filtered and cleaned. 
We use Semhash \citep{minishlab2025semhash} to perform exact de-duplication and semantic de-duplication on the data of NqOpen after filtering in step 1 to ensure data diversity. 
Exact de-duplication means excluding duplicate data in the dataset with exactly the same problem.
We use potion-base-8M \citep{minishlab2024model2vec} as the sentence embedding model for semantic de-duplication.
Based on the generated semantic vectors, we use the approximate nearest neighbor search algorithm to quickly search for similar vectors, mark the data with cosine similarity greater than a threshold as similar data and form a cluster, only one sample is selected from a cluster, and the rest of the data are marked as duplicate data and filtered. 
According to the entropy value calculated for each problem, the top 80\% proportion of data is selected as the filtered data, thus ensuring data diversity. 
Finally, the data from NqOpen after de-duplication and the filtered WebQuestions and ComplexQuestions data obtained in step 1 are combined to form the two-stage filtered data.

\paragraph{Refinement and Entity Extraction.}
In this step, we use the GPT-4O and predefined rules to check each question of the data obtained in step 2, to exclude questions that are not formal, do not have enough information to support reasoning about the answer, and are not formal in language. 
Carefully designed prompts enable the GPT-4O to accept or reject each data item, and for accepted items, to normalize, correct, and extract entities. 
Appendix shows the prompts used by the GPT-4O model for data filtering.

\paragraph{Difficulty Filtering.}
To avoid excessive difficulty in the training data, we choose to further filter the data obtained from the previous step using DeepSeek-R1, specifically selecting questions that DeepSeek-R1 answers correctly on its first attempt. 
This step also helped us get the long COT data needed for the SFT baseline.

\paragraph{Wikipedia-grounded Data Filtering.}
The goal of this step is to filter out data that cannot be matched to the corresponding knowledge from the Wikipedia knowledge source.
We use Wikipedia\footnote{20231101.en, \url{https://dumps.wikimedia.org/}.} (6.4 million entries) as our knowledge source. 
Based on each data item's entities, we retrieve corresponding Wikipedia entries and add their textual content as knowledge for the item into our knowledge base. An entity must exactly match a Wikipedia entry or be fully contained within a Wikipedia entry title for the match to be successful. 
To avoid redundancy, each entity keyword links to no more than three Wikipedia entries. 
Data items containing entities that do not match any Wikipedia entry are filtered out in this paper. 
Additionally, to ensure the stability of SFT training, we choose to retain only the 3,177 data items where DeepSeek-R1's output length is between 300 and 700 tokens as training data. 
So, We complete the filtering and construction of the training data.

\subsection{ColdStart Data Construction}
We obtain another part of the remaining data from NqOpen and perform the same filtering steps as we did to construct the RL training data.
We use DeepSeek-R1 to distill the long COT data and filter out the questions that DeepSeek-R1 answered correctly the first time. 
And merge the data that failed to match the knowledge in the RL training data construct as data source. 
Only 1798 data items with DeepSeek-R1 output length between 300 and 700 are kept as cold-start training data.






==> section_knowrl/preliminary.tex <==
\section{Preliminary}

In this paper, we chose to first use supervised fine-tuning for cold-start training of slow thinking models and then use the Grouped Relative Policy Optimization \citep[GRPO;][]{shao2024deepseekmath}) algorithm for reinforcement learning training. We will introduce SFT and reinforcement learning algorithms for language model fine-tuning.

SFT is a method for improving the ability of a model to follow instructions and adapt to specific downstream tasks by having the model parameters fit a high-quality dataset.
SFT aims to minimize the negative log-likelihood loss to maximize the conditional probability \( P_{\theta}(y|x) \) of generating the target sequence \( y \) given the input \( x \). For the entire dataset \( D \), the loss function \( L_{SFT} \) of SFT can be expressed as:
\begin{equation}
L_{SFT}(\theta) = -\sum_{(x,y) \in D} \log P_{\theta}(y|x).
\end{equation}
As \( L_{SFT} \) decreases continuously, the probability of the model generating the expected output given the input gradually increases. Using SFT as a cold-start training before reinforcement learning training can speed up the convergence of the reward curve during reinforcement learning training.

GRPO is a highly efficient reinforcement learning method that replaces traditional value network-based advantage estimation with a unique group relative reward mechanism. GRPO removes the value network found in traditional Proximal Policy Optimization \citep[PPO;][]{schulman2017proximal}, retaining only the policy network. This, to a certain extent, reduces computational and memory requirements.

The group relative reward mechanism in GRPO refers to sampling multiple candidate outputs (or actions) from the current prompt (or state) to form a "response group" (or action group). Then, by normalizing the rewards of the outputs within the group, a relative advantage value is obtained, thereby replacing traditional absolute advantage estimation. The GRPO objective function is constructed from two main components per timestep $t$.
First, the PPO-style clipped surrogate objective is defined as:
\begin{equation} \label{eq:grpo_clip}
L^{\text{CLIP}}_t(\theta) = \min(r_t(\theta)A_t, \text{clip}(r_t(\theta), 1-\epsilon, 1+\epsilon)A_t).
\end{equation}
Second, the gradient regularization term introduced by GRPO is:
\begin{equation} \label{eq:grpo_reg}
L^{\text{REG}}_t(\theta) = \lambda \|\nabla_\theta r_t(\theta)\|^2.
\end{equation}
The overall GRPO objective function, $L^{\text{GRPO}}(\theta)$, is then the expectation over timesteps $t$ of the difference between these two components:
\begin{equation} \label{eq:grpo_objective_final}
L^{\text{GRPO}}(\theta) = \mathbb{E}_t [L^{\text{CLIP}}_t(\theta) - L^{\text{REG}}_t(\theta)].
\end{equation}

The GRPO objective function, $L^{\text{GRPO}}(\theta)$ as defined in Equation~\eqref{eq:grpo_objective_final}, aims to improve the policy by optimizing the policy parameters $\theta$. It is an expectation over timesteps $t$.
The first component for each timestep, $L^{\text{CLIP}}_t(\theta)$ given by Equation~\eqref{eq:grpo_clip}, is the classic clipped surrogate objective from PPO. Within this term, $r_t(\theta)$ is the policy probability ratio, specifically $\frac{\pi_\theta(a_t|s_t)}{\pi_{\text{old}}(a_t|s_t)}$, which compares the probability of taking action $a_t$ in state $s_t$ under the current policy $\pi_\theta$ (determined by parameters $\theta$) versus the old policy $\pi_{\text{old}}$ (used to collect the data). $A_t$ represents the advantage function, which in GRPO specifically refers to the relative advantage value calculated via the group relative reward mechanism, quantifying how good the current action is. The $\text{clip}$ function constrains $r_t(\theta)$ to the range $[1-\epsilon, 1+\epsilon]$, where $\epsilon$ is a small hyperparameter used to limit the magnitude of policy updates, preventing excessively large updates that could destabilize training.
The second component for each timestep, $L^{\text{REG}}_t(\theta)$ from Equation~\eqref{eq:grpo_reg}, is the gradient regularization term introduced by GRPO. Here, $\nabla_\theta r_t(\theta)$ denotes the gradient of the policy probability ratio $r_t(\theta)$ with respect to the policy parameters $\theta$, and $\lambda$ is a regularization coefficient. This term, $L^{\text{REG}}_t(\theta)$, penalizes the L2 norm (squared) of the gradient of the policy probability ratio, further constraining the magnitude of policy updates. This helps prevent overly rapid policy changes and ensuing instability, which is particularly important for GRPO as it operates without the assistance of a value network. The final objective $L^{\text{GRPO}}(\theta)$ then combines these by taking the expectation of $L^{\text{CLIP}}_t(\theta) - L^{\text{REG}}_t(\theta)$.








==> tables/knowrl.tex <==
\definecolor{lightgreen}{HTML}{E6FFFA} 
\definecolor{tablehighlight}{HTML}{D5F5E3} 
\begin{table*}[h]
    \centering
    \small
    \setlength{\tabcolsep}{3.2pt}
    \renewcommand{\arraystretch}{1.2} % Slightly increase row height for readability
    \begin{tabular}{l|ccc|cc}
    \toprule
    \multirow{2}{*}{\makecell[c]{\normalsize\textbf{Methods}}} & \multicolumn{3}{c|}{\textbf{Hallucination}} & \multicolumn{2}{c}{\textbf{Reasoning}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-6}
    & \small\textbf{TruthfulQA} & \small\textbf{SimpleQA} & \small\textbf{ChineseSimpleQA}  & 
    \small\textbf{GPQA Diamond} & \small\textbf{AIME 2025}\\
   
    \midrule
    \multicolumn{6}{c}{\textbf{Skywork-OR1-7B-Preview}} \\
    \text{Direct Generation}     & 34.39 & 5.19 & 13.27  & 31.31 & 6.67  \\
    %\text{COT}                   & 35.01 & 5.11 & 9.50   & 39.90 & 23.33  \\
    \text{Self-Refine}           & 30.00 & 2.90 & 11.57  & 46.97 & 36.67 \\
    %\text{SC}                    & 34.64 & 6.34 & 15.77  & 41.41 & 26.67  \\
    \text{FactTune-FS}           & 34.76 & 5.33 & 12.30 & 32.83 & 6.67  \\
    \text{DPO}                   & 34.64 & 4.60 & 15.57 & 34.34 & 6.67 \\
    \text{SFT}                   & \textbf{38.43} & 4.90 & 14.87 & 32.32 & 16.67  \\
    %\midrule
    \rowcolor{tablehighlight} % Changed color here
    \text{KnowRL-Zero}           & 34.39 & \textbf{5.55} & 15.17 & 30.30 & 10.00  \\
    %\text{ColdStart}             & 35.99 & 5.14 & 14.67 & 33.84 & 20.00   \\
    %\text{ColdStart+SFT}         & 36.11 & 4.58 & 14.87 & 30.30 & 16.67 \\
    %\text{ColdStart+DPO}         & 32.68 & 4.53 & 11.77 & 36.36 & 13.33  \\
    \rowcolor{tablehighlight} % Changed color here
    \text{KnowRL}      & 37.70 & 4.58 & \textbf{16.23} & 34.34$\uparrow$ & 10.00$\uparrow$ \\
       
    \midrule
        \multicolumn{6}{c}{\textbf{DeepSeek-R1-Distill-Qwen-7B}} \\
    \text{Direct Generation}     & 33.05 & 1.92 & 11.17  & 34.34 & 16.67  \\
    %\text{COT}                   & 32.80 & 2.55 & 11.53  & 41.41 & 30.00  \\
    \text{Self-Refine}           & 33.90 & 2.60 & 9.97   & 45.45 & 33.33  \\
    %\text{SC}                    & 34.88 & 3.04 & 11.47  & 42.42 &  23.33 \\
    \text{FactTune-FS}           & 35.50 & 2.46 & 10.27 & 36.87 & 26.67  \\
    \text{DPO}                   & 36.96 & 3.21 & 12.33 & 37.37 & 13.33  \\
    \text{SFT}                   & 37.09 & 4.12 & 12.70 & 30.30 & 16.67    \\
    %\midrule
    \rowcolor{tablehighlight} % Changed color here
    \text{KnowRL-Zero}            & 33.54 & 1.34 & 11.00 & 34.34 & 6.67  \\
    %\text{ColdStart}             & 35.86 & 3.75 & 12.70 & 39.39 & 20.00   \\
    %\text{ColdStart+SFT}         & 37.21 & 3.59 & 13.47 & 31.31 & 16.67 \\
    %\text{ColdStart+DPO}         & 33.41 & 3.34 & 10.63 & 33.84 & 6.67  \\
    \rowcolor{tablehighlight} % Changed color here
    \text{KnowRL}      & \textbf{38.19} & \textbf{4.56} & \textbf{13.90} & 37.37$\uparrow$ &  13.33$\downarrow$ \\
    
    
    \bottomrule
    \end{tabular}
    \vspace{-1ex}
    \caption{\textbf{Main Experiment.} KnowRL-Zero is a method of RL training without cold-start training. KnowRL represents RL training on a cold-start trained model. The best results are marked in \textbf{bold}.}
    \vspace{-3ex}
    \label{main-exp}
\end{table*}

\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/rl_training_curves_comparison.pdf}
    % \vspace{-2ex}
    \caption{\textbf{KnowRL Training Curve.} The Combined Reward is $R_{combined}$.}
    \vspace{-3ex}
    \label{knowrl-exp}
\end{figure*}



\begin{table*}[t]
    \centering
    \small
    \setlength{\tabcolsep}{3.2pt}
    \renewcommand{\arraystretch}{1.2}
    % Define table structure: 3 cols for rewards, 3 for Hallucination, 2 for Reasoning
    \begin{tabular}{ccc|ccc|cc}
    \toprule
    % Main header row
    \multicolumn{3}{c|}{\textbf{Reward}} & \multicolumn{3}{c|}{\textbf{Hallucination}} & \multicolumn{2}{c}{\textbf{Reasoning}} \\
    \cmidrule(lr){4-6} \cmidrule(lr){7-8}
    % Sub-header row
    \textbf{$R_{format}$} & \textbf{$R_{fact}$} & \textbf{$R_{correct}$} & \small\textbf{TruthfulQA} & \small\textbf{SimpleQA} & \small\textbf{ChineseSimpleQA} &
    \small\textbf{GPQA Diamond} & \small\textbf{AIME 2025}\\

    \midrule
    \multicolumn{8}{c}{\textbf{DeepSeek-R1-Distill-Qwen-7B}} \\
   
    \checkmark & \ding{55} & \ding{55} & 33.41 & \textbf{2.36} & 10.47  & 35.86 & 10.00  \\
    \checkmark & \checkmark & \ding{55} & 34.03 & 1.55 & 9.70  & 31.31 & 16.67  \\
    \checkmark & \ding{55} & \checkmark & \textbf{34.76}  & 1.74 & 10.97 & \textbf{37.88} & \textbf{20.00}  \\
    \rowcolor{tablehighlight}
    \checkmark & \checkmark & \checkmark & 33.54 & 1.34 & \textbf{11.00} & 34.34 & 6.67  \\
        
    \midrule
    \multicolumn{8}{c}{\textbf{DeepSeek-R1-Distill-Qwen-7B-ColdStart}} \\
  
    \checkmark & \ding{55} & \ding{55} & 36.84 & 3.73 & 14.37 & 35.86 & \textbf{16.67}  \\
    \checkmark & \checkmark & \ding{55} & 37.82 & \textbf{6.16} & \textbf{14.60} & 35.86 & 13.33 \\
    \checkmark & \ding{55} & \checkmark & 37.82 & 4.04 & 13.80 & 33.33 & \textbf{16.67} \\
    \rowcolor{tablehighlight}
    \checkmark & \checkmark & \checkmark & \textbf{38.19} & 4.56 & 13.90 & \textbf{37.37} & 13.33 \\
    
    \bottomrule
    \end{tabular}
    \vspace{-1ex}
    \caption{\textbf{Reward Ablation Experiment.} DeepSeek-R1-Distill-Qwen-7B is trained with cold start to obtain DeepSeek-R1-Distill-Qwen-7B-ColdStart. The best results are marked in \textbf{bold}.
     For the reward components, \checkmark indicates inclusion and \ding{55} indicates exclusion.
    }
    \vspace{-3ex}
    \label{ablation}
\end{table*}


\begin{figure*}[t]
    \centering
     \vspace{2ex}
    \includegraphics[width=0.95\linewidth]{images/trainstep_two_models.pdf}
    \caption{Performance of the Skywork-OR1-7B-Preview and DeepSeek-R1-Distill-Qwen-7B on 5 datasets with different number of training steps.}
    \vspace{-4ex}
    \label{train-step1}
\end{figure*}



